Predicting post-release defects with knowledge units (KUs) of programming languages: an empirical study

Defect prediction plays a crucial role in software engineering, enabling developers to identify defect-prone code and improve software quality. While extensive research has focused on refining machine learning models for defect prediction, the exploration of new data sources for feature engineering remains limited. Defect prediction models primarily rely on traditional metrics such as product, process, and code ownership metrics, which, while effective, do not capture language-specific traits that may influence defect proneness. To address this gap, we introduce Knowledge Units (KUs) of programming languages as a novel feature set for analyzing software systems and defect prediction. A KU is a cohesive set of key capabilities that are offered by one or more building blocks of a given programming language. We conduct an empirical study leveraging 28 KUs that are derived from Java certification exams and compare their effectiveness against traditional metrics in predicting post-release defects across 8 well-maintained Java software systems. Our results show that KUs provide significant predictive power, achieving a median AUC of 0.82, outperforming individual group of traditional metric-based models. Among KU features, Method & Encapsulation, Inheritance, and Exception Handling emerge as the most influential predictors. Furthermore, combining KUs with traditional metrics enhances prediction performance, yielding a median AUC of 0.89. We also introduce a cost-effective model using only 10 features, which maintains strong predictive performance while reducing feature engineering costs. Our findings demonstrate the value of KUs in predicting post-release defects, offering a complementary perspective to traditional metrics. This study can be helpful to researchers who wish to analyze software systems from a perspective that is complementary to that of traditional metrics.

==> sections_jss/Bios.tex <==
\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/ahsan.jpg}}]
    {\scriptsize Md Ahasanuzzaman}\scriptsize is currently a Ph.D. student in the Software Analysis and Intelligence Lab (SAIL) at Queen's University, Canada. His research interests include mining software repositories (e.g., mobile app stores), source code analysis (e.g., mobile apps, Java applications), and machine learning. His studies got published in top Software Engineering venues (e.g., TSE, EMSE, and MSR). He obtained his BSc from the University of Dhaka in Bangladesh. He has been awarded prestigious awards, such as Deans scholarship award and Prime Minister Gold Medal for his outstanding achievements in the B.Sc program. More information at: \url{https://ahasanuzzaman.com/research/}
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/gus-bw.png}}]
	{\scriptsize Gustavo A. Oliva} \scriptsize is an Adjunct Professor at the School of Computing of Queen's University in Canada. Gustavo leads the blockchain research team at the Software Analysis and Intelligence Lab (SAIL). In addition to blockchain, he also conducts empirical studies in the fields of software ecosystems (e.g., npm), software evolution, and explanaible AI. Gustavo received his MSc and PhD degrees from the University of São Paulo (USP) in Brazil under the supervision of professor Dr. Marco Aur{é}lio Gerosa. More information at: \url{https://www.gaoliva.com}
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/ahmed.jpg}}]
    {\scriptsize Ahmed E. Hassan} \scriptsize is an IEEE Fellow, an ACM SIGSOFT Influential Educator, an NSERC Steacie Fellow, the Canada Research Chair (CRC) in Software Analytics, and the NSERC/BlackBerry Software Engineering Chair at the School of Computing at Queen’s University, Canada. His research interests include mining software repositories, empirical software engineering, load testing, and log mining. He received a PhD in Computer Science from the University of Waterloo. He spearheaded the creation of the Mining Software Repositories (MSR) conference and its research community. He also serves/d on the editorial boards of IEEE Transactions on Software Engineering, Springer Journal of Empirical Software Engineering, and PeerJ Computer Science. More information at: \url{http://sail.cs.queensu.ca}
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/jack.jpg}}] 
	{\scriptsize Zhen M. (Jack) Jiang} \scriptsize is an Associate Professor at the Department of Electrical Engineering and Computer Science, York University. Prior to joining York, he worked at BlackBerry Performance Engineering Team. His research interests lie within Software Engineering and Computer Systems. He is also the recipient of several best paper awards including ICST 2016, ICSE 2015 (SEIP track), ICSE 2013, WCRE 2011 and MSR 2009 (challenge track). Jack received his PhD from the School of Computing of Queen's University, Canada. He received his MSc from the University of Waterloo, Canada. More information at: \url{http://www.cse.yorku.ca/~zmjiang}
\end{IEEEbiography}

==> sections_jss/Conflict_Of_Interest.tex <==
\section*{Funding and/or Conflicts of interests/Competing interests}
\label{sec:Conflict_Of_Interest}
The authors declared that they have no conflict of interest.

==> sections_jss/Data_Availability_Statements.tex <==


\section*{Data Availability Statement (DAS)}
\label{sec:Data_Availability_Statement}

A supplementary material package is provided online in the following link:
\url{http://bit.ly/3GoSmHL}. The contents will be made available on a public GitHub
repository once the paper is accepted.

==> sections_jss/KU_Table.tex <==
\begin{table}[!htbp]
    \centering
    \caption{The identified Java programming language knowledge units (KUs).}
    \label{tab:topic_definition}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{3.2cm}p{13.8cm}}
        \toprule
        \multicolumn{1}{C{3cm}}{\textbf{Knowledge unit (KU)}} & \multicolumn{1}{C{14cm}}{\textbf{Definition}}                                                                                                                                                                                                                               \\ \midrule

        \textbf{[K1]} Data Type                                         &
        The declaration and initialization of different types of variables (e.g., primitive type and parameterized type.)
        \\ \midrule

        \textbf{[K2]} Operator and Decision                             &
        The usage of different Java operators (e.g., assignment, logical, and bit-wise operators) and conditional statements (e.g, if, if-else, and switch statements).
        \\ \midrule

        \textbf{[K3]} Array                                            &
        The declaration, instantiation, initialization and the usage of one-dimensional and multi-dimensional arrays.
        \\ \midrule

        \textbf{[K4]} Loop                                             &
        The execution of a set of instruction-s/methods repeatedly using for, while, and do-while statements and the skipping and stopping of a repetitive execution of instructions and methods using continue and break statements.
        \\ \midrule

        \textbf{[K5]} Method and Encapsulation                         &
        The creation of methods with parameters, the use of overloaded methods and constructors, the usage of constructor chaining, the creation of methods with variable length arguments, and the usage of different access modifiers. This KU also describes encapsulation mechanisms, such as creating a set and get method for controlling data access, generating immutable classes, and updating object type parameters of a method.
        \\ \midrule

        \textbf{[K6]} Inheritance                                      &
        Developing code with child class and parent class relationship, using polymorphism (e.g., developing code with overridden methods), creating abstract classes and interfaces, and accessing methods and fields of the parent's class.
        \\ \midrule

        \textbf{[K7]} Advanced Class Design                             &
        Developing code that uses the final keyword, creating inner classes including static inner classes, local classes, nested classes, and anonymous inner classes, using enumerated types including methods and constructors in an enum type, and developing code using @override annotator.
        \\ \midrule

        \textbf{[K8]} Generics and Collection                           &
        The creation and usage of generic classes, usage of different types of interfaces (e.g., List Interface, Deque Interface, Map Interface, and Set Interface), and comparison of objects using interfaces (e.g., java.util.Comparator, and java.lang.Comparable).
        \\ \midrule

        \textbf{[K9]} Functional Interface                         &
        The development of code that uses different versions of defined functional interfaces (e.g., primitive, binary, and unary) and user-defined functional interfaces.
        \\ \midrule

        \textbf{[K10]} Stream API                                       &
        The development of code with lambda expressions and Stream APIs. This includes developing code to extract data from an object using peek() and map() methods, searching for data with search methods (e.g., findFirst) of the Stream classes, sorting a collection using Stream API, iterating code with foreach of Stream, and saving results to a collection using the collect method.
        \\ \midrule

        \textbf{[K11]} Exception                                      &
        The creation of try-catch blocks, the usage of multiple catch blocks, the usage of try-with-resources statements, the invocation of methods throwing an exception, and the use of assertion for testing invariants.
        \\ \midrule

        \textbf{[K12]} Date time API                                   & This KU refers to create and manage date-based and time-based events using Instant, Period, Duration, and TemporalUnit, and work with dates and times across timezones and manage changes resulting from daylight savings, including Format date and times values. \\ \midrule

        \textbf{[K13]} IO                                              &
        Reading and writing data from console and files and using basic Java input-output packages (e.g., java.io.package).
        \\ \midrule

        \textbf{[K14]} NIO                                              &
        Interacting files and directories with the new non-blocking input/output API (e.g., using the Path interface to operate on file and directory paths). Performing other file-related operations (e.g., read, delete, copy, move, and managing metadata of a file or directory).
        \\ \midrule

        \textbf{[K15]} String Processing                                &
        The knowledge about searching, parsing, replacing strings using regular expressions, and using string formatting.
        \\ \midrule

        \textbf{[K16]} Concurrency                                      &
        The knowledge about functionalities that are related to thread execution and parallel programming. Some of these functionalities include: creating worker threads using Runnable and Callable classes, using an ExecutorService to concurrently execute tasks, using synchronized keyword and java.util.concurrent.atomic package to control the order of thread execution, using java.util.concurrent  classes and using a parallel fork/join framework.
        \\ \midrule

        \textbf{[K17]} Database                                        &
        The creation of database connection, submitting queries and reading results using the core JDBC API.
        \\ \midrule   

        \textbf{[K18]} Localization                                     &
        The knowledge about reading and setting the locale (Oracle defines a locale as ``a specific geographical, political, or cultural region'') by using the Locale object, and building a resource bundle for each locale, and loading a resource bundle in an application.
        \\ \midrule

        \textbf{[K19]} Java Persistence                                  &
        The usage of object/relational mapping facilities for managing relational data in Java applications. With this knowledge, developers can learn how to map, store, update and retrieve data from relational databases to Java objects and vice versa.                                                              \\ \midrule

        \textbf{[K20]} Enterprise Java Bean                             &
        The knowledge about managing server-side components that encapsulate the business logic of an application.                                                                                                                                                                                                               \\ \midrule

        \textbf{[K21]} Java Message Service API                         &
        The knowledge of how to create, send, receive and read messages using reliable, asynchronous, and loosely coupled communication.                                                                                                                                                                                                   \\ \midrule

        \textbf{[K22]} SOAP Web Service                               &
        Creating and using the Simple Object Access Protocol for sending and receiving requests and responses across the Internet using JAX-WS and JAXB APIs.                                                                                                                                                          \\ \midrule

        \textbf{[K23]} Servlet                                          &
        Handling HTTP requests, parameters, and cookies and how to process them on the server sites with appropriate responses.                                                                                                                                                                                           \\ \midrule

        \textbf{[K24]} Java REST API                                    &
        Creating web services and clients according to the Representational State Transfer architectural pattern using JAX-RS APIs.                                                                                                                                                                                     \\ \midrule

        \textbf{[K25]} Websocket                                         &
        Creating and handling bi-directional, full-duplex, and real-time communication between the server and the web browser.                                                                                                                                                                                         \\ \midrule

        \textbf{[K26]} Java Server Faces                                 &
        The knowledge about how to build UI component-based and event-oriented web interfaces using the standard JavaServer Faces (JSF) APIs.                                                                                                                                                                                                     \\ \midrule

        \textbf{[K27]} Contexts and Dependency Injection (CDI)             &
        Managing the lifecycle of stateful components using domain-specific lifecycle contexts and type-safely inject components (services) into client objects.                                                                                                                                                     \\ \midrule

        \textbf{[K28]} Batch Processing                                    &
        Creating and managing long-running jobs on schedule or on demand for performing on bulk-data, and without manual intervention.                                                                                                                                                                                 \\ \bottomrule
    \end{tabular}
    }
\end{table}

==> sections_jss/Preliminary_Study.tex <==
\section{Preliminary Study: \PrelimStudy}
\label{sec:Preliminary_Study}

\noindent \textbf{Motivation.} 
We compare KUs with traditional metrics. We conjecture that KUs provide a new perspective for the analysis of software code compared to traditional metrics.

\smallskip \noindent \textbf{Approach.} Our preliminary study is conducted in three steps, which are briefly explained below.

\begin{itemize}[label = \textbullet, itemsep=3pt, wide = 0pt, topsep=1pt, listparindent=\parindent]
	\item \textit{Step 1) Comparing KUs to traditional metrics via correlation analysis.} As a first step to determine how KUs and traditional metrics differ from one another, we calculate the Spearman's rank correlation coefficient ($rho$) between them. More formally, we calculate this correlation between all pairs of variables $x$ and $y$, where $x$ is a column in $D_{ku}$ and y is a column in $D_{cm}$. We choose the Spearman's $\rho$ in lieu of other correlation coefficients (e.g., Pearson's correlation) because the Spearman's $\rho$ does not require normally distributed data. We assess Spearman's $\rho$ using the following thresholds \citep{Evans95}, which operate on 2 decimal places only: \textit{very weak} for $|\rho| \leq 0.19$, \textit{weak} for $0.20 \leq |\rho| \leq 0.39$, \textit{moderate} for $0.40 \leq |\rho| \leq 0.59$, \textit{strong} for $0.60 \leq |\rho| \leq 0.79$, and \textit{large} for $|\rho| \geq 0.80$.

    \item \textit{Step 2) Clustering the files of the studied releases according to KUs and traditional metrics.} We first cluster the files of a project using KUs. Next, we re-cluster the files of the project using traditional metrics and evaluate how the two clusterings differ. We use the k-means clustering algorithm~\citep{comaniciu2002mean} to perform the clustering. K-means is one of the most popular clustering algorithms and has been widely used in software engineering research \citep{soft_fault_k_means, yoon_kmeans_soft_cluster, kmeans_software_cluster, cross_project_kmeans}. The detailed sub-steps are shown below:
    
    \begin{itemize}[itemsep=3pt, wide = 0pt, topsep=1pt, listparindent=\parindent]

		\item \textit{Step 2a) Reducing the dimensions of the datasets.} Many clustering algorithms (e.g., k-means algorithm) have inferior performance for high dimensional data ~\citep{parson_dimensionality}. To overcome the dimensionality issue, we reduce the dimension of our data using PCA before running the k-means algorithm. We perform the PCA on both KUs dataset $(Dataset(P,D_{ku}))$ and traditional metrics dataset $(Dataset(P,D_{cm}))$ of a project $P$ (see Section~\ref{sec:Data_Collection}) using the \texttt{PCA} class of scikit-learn package\footnote{\url{https://scikit-learn.org/dev/modules/generated/sklearn.decomposition.PCA.html}}. We reduce the dimension of our data by selecting the first-n PCA components that account for at least 90\% of the variance of the data.

        \item \textit{Step 2b) Identify optimal number of clusters.} The k-means algorithm takes the number of clusters as an input parameter (\textit{K}). To identify the optimal number of clusters, we analyze the \textit{silhouette} coefficient~\citep{rousseeuw1987silhouettes}. The silhouette coefficient is a popular measure that has been widely used in prior studies~\citep{nidheesh2020hierarchical, cluster_mobile_apps_ESEM_2016, clustering_text_lda_ICSE_2013} for determining the optimal number of clusters. The silhouette coefficient ranges from -1.0 to 1.0. A coefficient close to one indicates that the object well-matches its own cluster and, simultaneously, poorly-matches its neighboring clusters. If most objects have a high coefficient, then the clustering configuration is deemed appropriate. We run k-means for \textit{K} values ranging from 2 to 40 and calculate the \textit{mean silhouette} for each \textit{K} value.  We determine the optimal number of clusters by selecting the 
        \textit{K} that maximizes the mean silhouette score.

        \item \textit{Step 2c) Clustering the files of the studied releases.} To cluster the files of the studied releases using the k-means algorithm, we employ the \texttt{KMeans} class of scikit-learn from python\footnote{\url{https://scikit-learn.org/1.5/modules/generated/sklearn.cluster.KMeans.html}}. We use the selected PCA components as the input dataset. Finally, we cluster the studied releases using the k-means algorithm and visualize the clusters using the \texttt{fviz\_cluster} function of the \texttt{factoextra} R package~\citep{facto_extra}.

    \end{itemize}
    
	\item \textit{Step 3) Comparing the two clusterings.} We compare the two clusterings produced in the prior step. This comparison is done both visually and then statistically through the computation of the \textit{adjusted Rand index}. The Rand index refers to the probability that the two clusterings will agree on a randomly chosen pair of data points. The adjusted Rand index employs a correction-for-chance to the original Rand index. Intuitively, the adjusted Rand index is a measure of the similarity between two clusterings. The index ranges from zero (i.e., the two clusterings do not agree on any pair of points) to one (i.e., the clusterings are exactly the same).

	%To keep the paper organized and maintain its readability, we present the clustering results of a randomly selected project (the ``structurizr'' project) in this paper.
	
\end{itemize}
	
\smallskip \noindent \textbf{Findings.} \observation{The majority of KUs do not exhibit a strong correlation with traditional metrics.} Table~\ref{tab:strength_correlation_ku_code_metric} presents the strength of correlation between KUs and traditional metrics. We observe that no KUs show a large correlation with traditional metrics. We also observe that only 5.6\% of the identified KUs (e.g., Operator and Decision KU) show a strong a correlation with traditional metrics. However, the Spearman's $\rho$ for all pairs consisting of a traditional metrics and a KUs is below 0.60 for the majority of KUs (i.e., 94.4\% of the identified KUs).  Therefore, the majority of KUs do not exhibit a strong correlation with traditional metrics. This result indicates that KUs can provide an additional perspective for the analysis of software code.

\begin{table}[!t]
    \small
	\centering
	\caption{The strength of correlation between KUs and traditional metrics.}
	\label{tab:strength_correlation_ku_code_metric}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{lr}
	\toprule
	\multicolumn{1}{C{4.5cm}}{\textbf{Strength of correlation}} &
	\multicolumn{1}{C{3.5cm}}{\textbf{The percentage of KUs}}
	\\
	\midrule
	Large correlation ($|\rho| \ge 0.80$) & 0\% \\
	Strong correlation ($0.60 \le |\rho| \le 0.79$) & 5.6\% \\
	Moderate correlation ($0.40 \le |\rho| \le 0.59$) & 16.6\% \\
	Weak correlation ($0.20 \le |\rho| \le 0.39$) & 38.9\% \\
	Very weak correlation ($|\rho| \le 0.19$) & 38.9\%\\
	\bottomrule   
	\multicolumn{2}{l}{\pbox{9cm}{Here, $\rho$ denotes the Spearman correlation coefficient.}}
	\end{tabular}
	%}
	\end{table}

\begin{figure}[!h]
	\centering
	\includegraphics[width=1\linewidth]{./figures/RQ1/wicket-1.3.0-beta2.pdf}
	\caption{Identified clusters for knowledge units (KUs) and traditional metrics of the ``Wicket-1.3.0-beta2'' release.} 
	\label{fig:rq1_knowledge_code_cluster}
\end{figure}

\smallskip \observation{KUs identify two times more clusters than traditional metrics.} We observe that the clustering based on KUs produce 4 (median) clusters, whereas the clustering of traditional metrics produce e (median) clusters. In other words, the Java files of the studied releases can be seen as belonging to two times more clusters through the lens of KUs than the clusters that are identified by traditional metrics. Figure~\ref{fig:rq1_knowledge_code_cluster} depicts the identified clusters for KUs and traditional metrics for the ``Wicket-1.3.0-beta2''\footnote{\url{https://github.com/structurizr/java}}. We observe that the clustering based on the lens of KUs produce  4 clusters and traditional metrics produce 2 clusters.

Finally, we observe that the median value of \textit{adjusted Rand index} between the two clusterings across the studied releases is 0.54 which is lower than 1. In other words, the probability that the two clusterings will agree on a randomly chosen studied release is 54\% (after correction-for-chance adjustment). Since a Rand index value other than 1 indicates differences in clusters, we conclude that the clusters of KUs are not the same as those of traditional metrics.

\begin{figure}[!t]
	\centering
	\includegraphics[width=1.0\textwidth]{./figures/RQ1/wicket-1.3.0-beta2_cluster_overlap-cropped}
	\caption{Visualization of clusters for KUs and traditional metrics. Each polygon represents a cluster of KUs and the dotted points of colors represent files in the clusters of traditional metrics. } 
	\label{fig:rq1_overlap_knowledge_code_cluster}
\end{figure}

\smallskip \observation{The identified clusters via traditional metrics do not completely overlap with the identified clusters via KUs.} Figure~\ref{fig:rq1_overlap_knowledge_code_cluster} shows the overlap between the two clusterings of the ``Wicket-1.3.0-beta2'' project. Each polygon represents a cluster of KU and each colored point represents a file in one of the clusters of the traditional metrics clustering. As shown in Figure~\ref{fig:rq1_overlap_knowledge_code_cluster}, cluster 2, 3 and 4 of KUs (i.e., the polygons) contain files of different clusters of traditional metrics (i.e., each polygon contains different coloured points). For example, cluster 4 of KUs contains 25.0\% files of cluster 0 of traditional metrics and 75.0\% files of cluster 1 of traditional metrics. Therefore, these KU clusters are not completely overlapped by a single cluster of traditional metrics (i.e., a KU cluster contains files of more than one cluster of traditional metrics). This result is also an indication that KUs offer a complementary perspective for analyzing software code.

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\linewidth]{./figures/RQ1/ku_not_represent_cc_distr.pdf}
	\caption{The distribution of the percentage of KU clusters that are not overlapped by a single cluster of traditional metrics. } 
	\label{fig:rq1_per_ku_not_reprsent_by_single_code_cluster}
\end{figure}

Figure~\ref{fig:rq1_per_ku_not_reprsent_by_single_code_cluster} presents the distribution of the percentage of KU clusters that are not overlapped by a single cluster of traditional metrics across the studied releases. The median of the percentage of KU clusters that are not overlapped by a single traditional metrics cluster is 81.67\%, indicating that code clusters do not completely overlap with the KU clusters (i.e., polygons have a somewhat mix of different colored dots). Such a result indicates that there exists KU clusters that are not uniquely described by a single cluster of traditional metrics. This result is also an indication that KU clusters can capture a different perspective of software systems from the identified clusters via traditional metrics.

\begin{footnotesize}
    \begin{mybox}{Summary}
    	\textbf{Preliminary Study: \PrelimStudy}
        \tcblower
        KUs offer a new lens through which the code of software systems can be analyzed, revealing a perspective that is complementary to that yielded by traditional metrics. In particular:
    	\begin{itemize}[itemsep = 0pt, label=\textbullet, wide = 0pt]
    		
            \item None of the KUs exhibit a large correlation with traditional metrics.

    		\item Through the lens of KUs, the files of the studied projects could be grouped into two times more cluster than the identified clusters via traditional metrics.
    		
    		\item The identified clusters using traditional metrics do not completely overlap with the identified clusters using KUs.
    		
    	\end{itemize}
    \end{mybox}
\end{footnotesize}

==> sections_jss/temp.tex <==
\begin{itemize}[label = \textbullet, itemsep=3pt, wide = 0pt, topsep=1pt, listparindent=\parindent]
	\item \textit{Step 1) Comparing KUs to code metrics via correlation analysis.} As a first step to determine how KUs and code metrics differ from one another, we calculate the Spearman's rank correlation coefficient ($rho$) between them. More formally, we calculate this correlation between all pairs of variables $x$ and $y$, where $x$ is a column in $D_{ku}$ and y is a column in $D_{cm}$. We choose the Spearman's $\rho$ in lieu of other correlation coefficients (e.g., Pearson's correlation) because the Spearman's $\rho$ does not require normally distributed data. We assess Spearman's $\rho$ using the following thresholds \citep{Evans95}, which operate on 2 decimal places only: \textit{very weak} for $|\rho| \leq 0.19$, \textit{weak} for $0.20 \leq |\rho| \leq 0.39$, \textit{moderate} for $0.40 \leq |\rho| \leq 0.59$, \textit{strong} for $0.60 \leq |\rho| \leq 0.79$, and \textit{large} for $|\rho| \geq 0.80$.


	\item \textit{Step 2) Clustering the files of the studied projects according to KUs and code metrics.} We first cluster the files of a project using KUs. Next, we recluster the files of the project using code metrics and evaluate how the two clusterings differ. We use the k-means clustering algorithm~\citep{comaniciu2002mean} to perform the clustering. K-means is one of the most popular clustering algorithms and has been widely used in software engineering research \citep{soft_fault_k_means, yoon_kmeans_soft_cluster, kmeans_software_cluster, cross_project_kmeans}. The detailed sub-steps are shown below:

	\begin{itemize}[itemsep=3pt, wide = 0pt, topsep=1pt, listparindent=\parindent]

		\item \textit{Step 2a) Reducing the dimensions of the datasets.} Many clustering algorithms (e.g., k-means algorithm) have inferior performance for high dimensional data ~\citep{parson_dimensionality}. To overcome the dimensionality issue, we reduce the dimension of our data using PCA before running the k-means algorithm.
		
		We perform the PCA on both KUs dataset $(Dataset(P,D_{ku}))$ and code metric dataset $(Dataset(P,D_{cm}))$ of a project $P$ (see Section~\ref{sec:Data_Collection}) using the \texttt{PCA} class of scikit-learn package\footnote{\url{https://scikit-learn.org/dev/modules/generated/sklearn.decomposition.PCA.html}}. We reduce the dimension of our data by selecting the first-n PCA components that account for at least 90\% of the variance of the data. 

        \item \textit{Step 2b) Identify optimal number of clusters.} The k-means algorithm takes the number of clusters as an input parameter (\textit{K}). To identify the optimal number of clusters, we analyze the \textit{silhouette} coefficient~\citep{rousseeuw1987silhouettes}. The silhouette coefficient is a popular measure that has been widely used in prior studies~\citep{nidheesh2020hierarchical, cluster_mobile_apps_ESEM_2016, clustering_text_lda_ICSE_2013} for determining the optimal number of clusters. The silhouette coefficient ranges from -1.0 to 1.0. A coefficient close to one indicates that the object well-matches its own cluster and, simultaneously, poorly-matches its neighboring clusters. If most objects have a high coefficient, then the clustering configuration is deemed appropriate. 
		
		We run k-means for \textit{K} values ranging from 2 to 40 and calculate the \textit{mean silhouette} for each \textit{K} value.  The optimal number of clusters is determined by selecting the 
        \textit{K} that maximizes the mean silhouette score.

		\item \textit{Step 2b) Clustering the files of the studied projects.} To cluster the files of the studied releases using the k-means algorithm, we employ the KMeans class of scikit-learn from python  \footnote{\url{https://scikit-learn.org/1.5/modules/generated/sklearn.cluster.KMeans.html}. We use the selected PCA components as the input dataset. Finally, we cluster the studied releases using the k-means algorithm and visualize the clusters using the \texttt{fviz\_cluster} function of the \texttt{factoextra} R package~\citep{facto_extra}.
		 
	\end{itemize}

	\item \textit{Step 3) Comparing the two clusterings.} We compare the two clusterings produced in the prior step. This comparison is done both visually and then statistically through the computation of the \textit{adjusted Rand index}. The Rand index refers to the probability that the two clusterings will agree on a randomly chosen pair of data points. The adjusted Rand index employs a correction-for-chance to the original Rand index. Intuitively, the adjusted Rand index is a measure of the similarity between two clusterings. The index ranges from zero (i.e., the two clusterings do not agree on any pair of points) to one (i.e., the clusterings are exactly the same).

	%To keep the paper organized and maintain its readability, we present the clustering results of a randomly selected project (the ``structurizr'' project) in this paper.
	
\end{itemize}
